Testing of Autonomous Driving Systems: Where Are We and Where Should We Go?

Autonomous driving has shown great potential to reform modern transportation. Yet its reliability and safety have drawn a lot of attention and concerns. Compared with traditional software systems, autonomous driving systems (ADSs) often use deep neural networks in tandem with logic-based modules. This new paradigm poses unique challenges for software testing. Despite the recent development of new ADS testing techniques, it is not clear to what extent those techniques have addressed the needs of ADS practitioners. To fill this gap, we present the first comprehensive study to identify the current practices and needs of ADS testing. We conducted semi-structured interviews with developers from 10 autonomous driving companies and surveyed 100 developers who have worked on autonomous driving systems. A systematic analysis of the interview and survey data revealed 7 common practices and 4 emerging needs of autonomous driving testing. Through a comprehensive literature review, we developed a taxonomy of existing ADS testing techniques and analyzed the gap between ADS research and practitioners' needs. Finally, we proposed several future directions for SE researchers, such as developing test reduction techniques to accelerate simulation-based ADS testing.

==> Paper_Sections/6_gaps_back.tex <==
\section{Literature Review and Research Gaps} \label{sec:future}

The previous section summarizes four emergent needs from industrial practitioners in ADS testing based on interviews and surveys. To understand how and to what extent research from the SE community has addressed these needs, we surveyed research papers from SE conferences and journals and examined to what extent each need is addressed by state-of-the-art research.
\jz{
to-do:
1. figure 7, simulation testing replaced, replaced rote typo
2. replace coverage-based with knowledge-guided (restricted to one paragraph)
3. need 2 has now coverage-based metrics (moved over)
4.  Prima needs to associatd with confidence-based metric
5.  CV [132] future direction for knowledge-guided, summarize the technical details in 1-2 sentences
6.  Need 3 new paper covered
7. Need 4 restored
}









% \begin{table*}[]
% \caption{A taxonomy of ADS testing research.}
% \label{tab:ADS_papers}
% \vspace{-5pt}
% \centering
% \begin{tabular}{l|l|r|l}
% \hline
% \textbf{Category}                 & \textbf{Sub-category}         & \textbf{Paper count} & \textbf{Papers} \\ \hline
% Corner cases Generation           & Search-based Testing          & 12                                        & \cite{kluck2019genetic,  Ben_Abdessalem_2016testing, abdessalem2018testing, Gambi_2019automatically, Calo_2020generating, cal2020simulaneously, han2020metamorphic, li2020avfuzzer, mullins2018adaptive, riccio2020model, Abdessalem_2018testing, Gladisch_2019experience}            \\
%                                   & Adversarial Space             & 0                                        & None           \\
%                                   & Coverage-based Methods        & 2                                        & \cite{pei2017deepxplore, tian2018deeptest}            \\ \hline
% Test Selection and Prioritization & coverage-based metrics        & 2                                        & \cite{pei2017deepxplore, tian2018deeptest}           \\
%                                   & confidence-based metrics      & 0                                        & None            \\
%                                   & similarity-based test metrics & 0                                        & None            \\ \hline
% DSLs                              &                               & 1                                        & \cite{gambi2019generating}            \\ \hline
% Automated data processing         & Labeling                      & 0                                        & None            \\
%                                   & Cleaning                      & 0                                        & None\\ \hline
% Others                            &                               & 23                                        & \cite{simos2020importance, Kim_2019, zhang2018deeproad, han2020metamorphic, li2020avfuzzer, l12020ontology, zhou2018deepbillboard, secci2020on, wolschke2017observation, Knauss_2017software, Moukahal_2019security, Salay_2019A, Tobias_2018safety, Gustavsson_2016verification, Zhao_2019assessing, Kang_2017model, Abdessalem_2020sutomated, garcia2020comprehensive, Zhao_2020A, Jahangirova_2020An, Haq_2020comparing, Liu_2021An, King_2019automated}            \\ \hline
% \end{tabular}
% \end{table*}



%  \begin{figure*}[tb]
%     \centering
%     \includegraphics[width = 1\textwidth]{images/taxonomy.pdf}
%     \caption{A taxonomy of ADS testing research.}
%     \label{fig:ADS_papers}
% \end{figure*}


 \begin{figure*}[tb]
    \centering
    \includegraphics[width = 1\textwidth]{images/ADS Testing 2 (16).png}
    \caption{A taxonomy of ADS testing research.}
    \label{fig:ADS_papers}
\end{figure*}

\subsection{Literature taxonomy}
\label{sec:taxonomy}
% We divided papers about ADS testing into three categories as shown in %Table~\ref{tab:ADS_papers}
% \change{Figure~\ref{fig:ADS_papers}}. Papers belonging to test criteria introduced testing coverage metrics to evaluate the performance of ADSs and the quality of test cases. For testing case generation, several testing methods such as metamorphic testing, fuzzing testing, and search-based testing were applied in literature to generate testing scenarios of ADS. In addition, some empirical study were conducted in existing work to either analyze the security problems of ADS or evaluate the effectiveness of different testing methods and testing scenarios.

% We also summarized the research target and experiment environment of ADS testing papers. It can be seen that existing work in 7 out 9 subcategories focus on E2E ADS testing. For experiment environment, both real-world dataset and simulation environment are considered in research. 

\todo{expand the discussion here. Write at least 3 paragraphs.}
% We divided papers about ADS testing into five categories as shown in Figure~\ref{fig:ADS_papers}. Half of the related papers focus on corner case generation, and search-based methods and knowledge-based methods each make up half of them. Simulation testing is also an important research direction of ADS testing, while there are three papers discuss the potential issues in simulation platforms, and another three works focus on the design and usage of simulation platforms. Furthermore, there are also some studies trying to use test selection and test prioritization in the field of autonomous driving to improve test efficiency. In addition, there is also some papers that survey specific parts of the ADS test. Papers that are not related to the industrial needs discussed in this article are classified as others. \todo{How about survey}



\change{We surveyed research papers from $28$ SE conferences, journals and workshops including ICSE, ESEC/FSE, ASE, ISSTA, ISSRE, ICST, QRS, TSE, JSS, and IST. Our goal is to find research papers that may propose potential solutions for the challenges and needs of testing ADS as identified in our interview and survey. Specifically, we used $35$ keywords including \texttt{autonomous driving}, \texttt{autonomous vehicle}, \texttt{traffic scene}, and \texttt{Apollo} to identify research papers related to autonomous driving. We implemented a crawler to download these papers from their publisher websites and found \AllNumber papers that contain at least one of the keywords in their title or abstract. By manually reviewing these papers, we identified \ADSAndTestingNumber papers related to ADS. Among them, \ADSTestingNumber papers are high related to ADS testing. We further manually categorized these \ADSTestingNumber ADS testing papers into different categories and sub-categories based on their research questions and solutions, as shown in Figure~\ref{fig:ADS_papers}.} \todo{check number}

\change{The right side of the Figure~\ref{fig:ADS_papers} illustrates 24 SE papers which help to address emerging needs discussed in Section~\ref{sec:needs}. These SE papers focus on two directions: \textit{Corner Case Generation} and \textit{Test Selection and Prioritization}. 22 papers on \textit{Corner Case Generation} are further classified according to the generation methods in to \textit{Search-based} and \textit{Knowledge-based} methods. The detailed analysis of how these papers can be used to solve those emerging needs is discussed in Section~\ref{sec:Need1GF}. For \textit{Test Selection and Prioritization papers}, all of 3 papers use \textit{similarity-based} methods, and are discussed in Section~\ref{sec:need2_solution}. For paper~\cite{li2020av}, as it not only generates corner cases, but also apply test prioritization techniques, it is included in both categories.}

\change{The left side of the Figure~\ref{fig:ADS_papers} shows 16 SE papers that are not related to these 4 emerging needs but are still researching ADS testing. Among them, there are 4 \textit{Survey} papers focusing on the potential bugs of ADS~\cite{}, the challenges of ADS testing~\cite{}, test scenarios~\cite{} and test metrics~\cite{}. Papers focusing on directions that not related to emerging needs, such as ADS formal verification~\cite{fritzsch2021experiences, du2021towards} and drawbacks of simulation tools~\cite{masuda2017software, hu2021disclosing}, are classified as \textit{Others}.}
% 22 papers focus on corner case generation in ADS testing. 



% Half of the related papers focus on corner case generation, and search-based methods and knowledge-based methods each make up half of them. Simulation testing is also an important research direction of ADS testing, while there are three papers discuss the potential issues in simulation platforms, and another three works focus on the design and usage of simulation platforms. Furthermore, there are also some studies trying to use test selection and test prioritization in the field of autonomous driving to improve test efficiency. In addition, there is also some papers that survey specific parts of the ADS test. Papers that are not related to the industrial needs discussed in this article are classified as others.

% Papers belonging to test criteria introduced testing coverage metrics to evaluate the performance of ADSs and the quality of test cases. For testing case generation, several testing methods such as metamorphic testing, fuzzing testing, and search-based testing were applied in literature to generate testing scenarios of ADS. In addition, some empirical study were conducted in existing work to either analyze the security problems of ADS or evaluate the effectiveness of different testing methods and testing scenarios.

% We also summarized the research target and experiment environment of ADS testing papers. It can be seen that existing work in 7 out 9 subcategories focus on E2E ADS testing. For experiment environment, both real-world dataset and simulation environment are considered in research. 

















% \subsection{Gaps and Future Directions for Need 1}
% \label{sec:Need1GF}
% Corner cases in ADSs are thought as safety-critical driving scenarios that are rare in the real world and possibly cause traffic accidents (e.g., collision).
% As discussed in section~\ref{sec:need1}, %in industry, 
% the de facto way to find corner cases in the industry is to conduct long hours of on-road testing.
% However, this method is time-consuming and expensive.

% The SE community has investigated a variety of methods to generate corner cases for ADSs. One common method is \textbf{search-based method}~\cite{gambi2019asfault, luo2021targeting, tang2021systematic, gladisch2019experience, ishikawa2020testing, borg2021digital, yin2021analyzing, laurent2021achieving, coletti2021diagnosing, calo2020simultaneously, abdessalem2018vision, gambi2019automatically, calo2020generating}.
% Search-based method aims to find a set of testing parameters in a parameter search space to identify %testing scenarios that are most likely to cause collision. 
% safety-critical scenarios, including collision and lane departure.
% The search process is normally guided by manually defined fitness functions such as time-to-collision and minimal distance between the ego-vehicle and pedestrians. \change{Optimal solutions of such fitness functions are usually found by applying genetic algorithms~\cite{gambi2019asfault, luo2021targeting, yin2021analyzing, abdessalem2018vision, gambi2019automatically} and Bayesian optimization~\cite{gladisch2019experience}.}
% AsFault~\cite{gambi2019asfault} uses genetic algorithms to evaluate parameters of road, like length and position, to make the ego-vehicle more error-prone on lane keeping task on generated test cases.
% These methods require prior knowledge to define a proper search space and fitness function. However, given the variety and complexity of real-world driving scenarios, it is challenging to pre–define a tractable search space. \change{Currently, as shown in Figure~\ref{fig:ADS_papers}, existing SE work mainly test on single module of ADS, including collision avoidance~\cite{tang2021systematic, calo2020generating, yin2021analyzing}, route planning~\cite{luo2021targeting, ishikawa2020testing, laurent2021achieving, coletti2021diagnosing, calo2020simultaneously, gambi2019automatically} and lane keeping~\cite{gambi2019asfault}, participants detection~\cite{borg2021digital}}. In SE community, there are some papers providing ideas for expanding the search space with additional materials. \todo{check module 是不是可以}
% % These methods require prior knowledge to define a proper search space and fitness function. Given the variety and complexity of real-world driving scenarios, it is challenging to pre–define a tractable search space. It is also challenging to search for the unknowns. 
% Wang et al.~\cite{wang2020automatic} explored how to mine new requirements and corresponding formal constraints from use case specifications using NLP techniques for cyber-physical systems. Gambi et al.~\cite{gambi2019generating} explored how to generate driving scenarios from historical crash reports. As a future direction, it is worth investigating how to elicit new safety requirements from existing crash reports, traffic rules and on-road driving recordings. Such requirements can be used to generate new fitness functions or refine existing ones to augment the search space for more mission-critical testing scenarios. 

% % Another type of corner cases generation explores the {\bf adversarial space} from existing testing data to mislead a model to make wrong predictions~\cite{goodfellow2014explaining, szegedy2013intriguing}. Wang et al.~\cite{wang2021advsim} used a new adversarial cost function to apply perturbations on input data to generate collision-prone trajectories. The cost function combines a trajectory cost, a collision cost and a safety cost to generate adversarial trajectories for a multi-module driving system. These unsafe trajectories are then implemented by modifying existing real LiDARs sweeps to generate feasible collision scenarios. Similarly, Mouret et al.~\cite{mouret2015illuminating} presented an approach that utilizes illumination search to identify an optimal feature map. This feature map is then used to generate corner cases to test a lane keeping assistant system. These methods require either prior knowledge to define the required evaluation metrics (e.g, standard deviation of the steering angle) or are restricted to single-modal sensor (LiDAR). As future work, new {\bf adversarial space} search algorithms are needed to allow exploring dangerous traffic scenarios with multi-modal sensor input data~\cite{daab2019feature, li2019aads}. Another promising line of work is to use geometry-aware adversarial cost function to generate corner-case scenarios, which is more suitable for the underlying sensor data~\cite{wen2019geometry}.
% % \todo{It is same with search based}

% \jz{
% to-do:
% 1. knowledge-based: existing work describe technical summary in terms of knowledge
% 2. Change DeepTest -> malfunctioning camera, not talk about neuron coverage. Align with knowledge
% 3. Future: 98 CV talk about technical points
% }
% \change{Furthermore, \textbf{Knowledge-based methods}~\cite{zhang2018deeproad, tian2018deeptest, valle2021metamorphic, zhou2020deepbillboard, han2020metamorphic, gambi2019generating, li2020av, kluck2018using, chandrasekaran2021combinatorial, tao2019industrial, gambi2019reconstructing} are widely explored in the SE community. According to Figure~\ref{fig:ADS_papers}, 2 papers testing on ADS functions, and 9 papers focus on system level ads testing. Among these 9 papers, 3 of them test on multi-modual ADS, such as Simulink~\cite{valle2021metamorphic} and Apollo~\cite{han2020metamorphic, li2020av}, while other 6 of them focus on the end-to-end ADS~\cite{zhang2018deeproad, tian2018deeptest, zhou2020deepbillboard, gambi2019generating, chandrasekaran2021combinatorial, gambi2019reconstructing}. 
% Different from search-based methods, knowledge-based methods generate corner cases from human knowledge, including driving experience, traffic accident reports, traffic law and regulations, rather than searching from the input space.
% Gambi et al.~\cite{gambi2019generating} extract safety-critical driving scenarios from police crash report. DeepTest~\cite{tian2018deeptest} generates corner cases using the metamorphic relation from driving experience that minor defacement of image inputs should not affect the steering of ADS.
% % DeepTest~\cite{tian2018deeptest} used neuron coverage to identify road images that maximize erroneous behaviors of a driving model. 
% % DeepRoad extended DeepTest to generate more natural road images using GAN~\cite{zhang2018deeproad}. 
% % Yet it need to be trained on a large amount of training data and is limited to simple transformations such as changing sunny weather to rainy weather. 
% The SE community should explore more advanced CV techniques such as~\cite{huang2018multimodal} to more effectively generate complex and realistic driving data. Moreover, existing work targets mainly at single-modal and simple end-to-end driving systems. As a future work, more systematic coverage-based research needs to be conducted to generate realistic driving scenes for multi-module and multi-modal ADSs.
% \lou{Possibile Direction 1: multi-module, 2:}
% } 

% Furthermore, \textbf{coverage-based methods}~\cite{pei2017deepxplore, tian2018deeptest} are widely explored in the SE community. Coverage-based methods rely on the notion of neuron coverage~\cite{pei2017deepxplore} and its variants~\cite{ma2018deepgauge, hu2019deepmutation}. These methods assume that a test case with higher neuron coverage can expose more erroneous behaviors of a DNN model. DeepXplore~\cite{pei2017deepxplore} used a gradient-based search method to find inputs that maximize neuron coverage and cause inconsistent behaviors among multiple DNN systems. DeepTest~\cite{tian2018deeptest} used neuron coverage to identify road images that maximize erroneous behaviors of a driving model. 
% Harel-Canada et al.~\cite{harel2020neuron} showed that higher neuron coverage actually leads to fewer defects detected and less natural inputs. DeepRoad extended DeepTest to generate more natural road images using GAN~\cite{zhang2018deeproad}. Yet it need to be trained on a large amount of training data and is limited to simple transformations such as changing sunny weather to rainy weather. The SE community should explore more advanced CV techniques such as~\cite{huang2018multimodal} to more effectively generate complex and realistic driving data. Moreover, existing work targets mainly at single-modal and simple end-to-end driving systems. As a future work, more systematic coverage-based research needs to be conducted to generate realistic driving scenes for multi-module and multi-modal ADSs.




\subsection{Gaps and Future Directions for Need 1}
\label{sec:Need1GF}
Corner cases in ADSs are thought as safety-critical driving scenarios that are rare in the real world and possibly cause traffic accidents (e.g., collision).
As discussed in section~\ref{sec:need1}, %in industry, 
the de facto way to find corner cases in the industry is to conduct long hours of on-road testing.
However, this method is time-consuming and expensive.
The SE community has investigated a variety of methods to generate corner cases for ADSs.
\jz{todo:
1. change the figure 7 taxonomy. remove 41 & 10 category; move coverage-based back to corner case generation; replace knowledge-based with coverage-based;  Coverage-based has two subcatogries: Neuron coverage; Scenario Coverage.
2. Gap 1: Leveraging scenario-based coverage and code-based coverage for ADS is promising.  There are a few works utilizing ontology for corner-case generation (e.g., crash report []). However, these ontologies are either too simple or pre-defined.  There are diverse and changing traffic rules and regulations, a self-evolving ontology utilizing NLP might be promising to encapsulate such regulations to generate more corner cases.
}


One common method is the \textbf{Knowledge-based method}~\cite{zhang2018deeproad, tian2018deeptest, valle2021metamorphic, zhou2020deepbillboard, han2020metamorphic, gambi2019generating, li2020av, kluck2018using, chandrasekaran2021combinatorial, tao2019industrial, gambi2019reconstructing}. 
Currently, knowledge-based methods are widely studied on different kinds of ADS in SE community. 
% According to Figure~\ref{fig:ADS_papers}, 2 papers testing on ADS functions, and 9 papers focus on system level ads testing. Among these 9 papers, 3 of them test on multi-modual ADS, such as Simulink~\cite{valle2021metamorphic} and Apollo~\cite{han2020metamorphic, li2020av}, while other 6 of them focus on the end-to-end ADS~\cite{zhang2018deeproad, tian2018deeptest, zhou2020deepbillboard, gambi2019generating, chandrasekaran2021combinatorial, gambi2019reconstructing}. 
\change{Generally speaking, knowledge-based methods generate corner cases using domain specific ontology and metamorphic relations extracted from human knowledge, including driving experience, traffic accident reports, traffic law and regulations.}
DeepTest~\cite{tian2018deeptest} and DeepRoad~\cite{zhang2018deeproad} generate corner cases using the metamorphic relation from driving experience that minor defacement of image inputs and weather changes should not affect the steering of ADS.
AC3R~\cite{gambi2019generating} uses domain-specific ontology and natural language processing techniques to extract information from police crash reports, to reconstruct corner cases of crash accidents. 
However, as discussed in Section~\ref{sec:need1}, driving scenarios are complicated, and it is difficult for human knowledge to cover all corner cases.

% Gambi et al.~\cite{gambi2019generating} extract safety-critical driving scenarios from police crash report. DeepTest~\cite{tian2018deeptest} generates corner cases using the metamorphic relation from driving experience that minor defacement of image inputs should not affect the steering of ADS.



\change{The \textbf{search-based methods}~\cite{gambi2019asfault, luo2021targeting, tang2021systematic, gladisch2019experience, ishikawa2020testing, borg2021digital, yin2021analyzing, laurent2021achieving, coletti2021diagnosing, calo2020simultaneously, abdessalem2018vision, gambi2019automatically, calo2020generating} are potentially to solve such kind problem.}
Search-based method aims to find a set of testing parameters in a parameter search space to identify safety-critical scenarios, including collision and lane departure. 
For the parameter search space, most paper focus on driving patterns, which is design based on states of the autonomous vehicle, such as the position and speed, and traffic participants.
The search process is normally guided by manually defined fitness functions such as time-to-collision and minimal distance between the ego-vehicle and pedestrians. 
\change{Optimal solutions of such fitness functions are usually found by applying genetic algorithms~\cite{gambi2019asfault, luo2021targeting, yin2021analyzing, abdessalem2018vision, gambi2019automatically} and Bayesian optimization~\cite{gladisch2019experience}.}
AsFault~\cite{gambi2019asfault} uses genetic algorithms to evaluate parameters of road, like length and position, to make the ego-vehicle more error-prone on lane keeping task on generated test cases.
\change{Because search-based methods traverse all parameters of the search space, it is more likely to find corner cases than knowledge-based methods. However, }These methods require prior knowledge to define a proper search space and fitness function. 
Given the variety and complexity of real-world driving scenarios, it is also challenging to pre–define a tractable search space. 
% \change{Currently, as shown in Figure~\ref{fig:ADS_papers}, existing SE work mainly test on single module of ADS, including collision avoidance~\cite{tang2021systematic, calo2020generating, yin2021analyzing}, route planning~\cite{luo2021targeting, ishikawa2020testing, laurent2021achieving, coletti2021diagnosing, calo2020simultaneously, gambi2019automatically} lane keeping~\cite{gambi2019asfault} and participants detection~\cite{borg2021digital}}. 
In SE community, there are some papers providing ideas for expanding the search space with additional materials.
% These methods require prior knowledge to define a proper search space and fitness function. Given the variety and complexity of real-world driving scenarios, it is challenging to pre–define a tractable search space. It is also challenging to search for the unknowns. 
Wang et al.~\cite{wang2020automatic} explored how to mine new requirements and corresponding formal constraints from use case specifications using NLP techniques for cyber-physical systems. 
%Gambi et al.~\cite{gambi2019generating} explored how to generate driving scenarios from historical crash reports. 
As a future direction, it is worth investigating how to elicit new safety requirements from existing crash reports, traffic rules and on-road driving recordings. Such requirements can be used to generate new fitness functions or refine existing ones to augment the search space for more mission-critical testing scenarios. 

% Another type of corner cases generation explores the {\bf adversarial space} from existing testing data to mislead a model to make wrong predictions~\cite{goodfellow2014explaining, szegedy2013intriguing}. Wang et al.~\cite{wang2021advsim} used a new adversarial cost function to apply perturbations on input data to generate collision-prone trajectories. The cost function combines a trajectory cost, a collision cost and a safety cost to generate adversarial trajectories for a multi-module driving system. These unsafe trajectories are then implemented by modifying existing real LiDARs sweeps to generate feasible collision scenarios. Similarly, Mouret et al.~\cite{mouret2015illuminating} presented an approach that utilizes illumination search to identify an optimal feature map. This feature map is then used to generate corner cases to test a lane keeping assistant system. These methods require either prior knowledge to define the required evaluation metrics (e.g, standard deviation of the steering angle) or are restricted to single-modal sensor (LiDAR). As future work, new {\bf adversarial space} search algorithms are needed to allow exploring dangerous traffic scenarios with multi-modal sensor input data~\cite{daab2019feature, li2019aads}. Another promising line of work is to use geometry-aware adversarial cost function to generate corner-case scenarios, which is more suitable for the underlying sensor data~\cite{wen2019geometry}.
% \todo{It is same with search based}

\jz{
to-do:
1. knowledge-based: existing work describe technical summary in terms of knowledge
2. Change DeepTest -> malfunctioning camera, not talk about neuron coverage. Align with knowledge
3. Future: 98 CV talk about technical points
}






\subsection{Gaps and Future Directions for Need 2} \label{sec:need2_solution}

As discussed in Section~\ref{sec:need2}, on-road testing is a time-consuming process. While simulation testing is used as an alternative, industrial practitioners find it still not sufficient. For this need of speeding up ADS testing, one promising direction the SE community can contribute to is test selection and prioritization. That is, SE researchers can develop techniques that ignore repetitive testing scenarios in the driving data and prioritize test cases that are more likely to expose errors in an ADS. For example, when driving on highway, the ego-vehicle often goes straight on a specific lane at a constant speed. Therefore, there is no need to replay the entire highway driving recording but only unique driving scenarios during the recording, such as lane cutting. 


%Currently, there is little discussion of test selection and prioritization in ADS testing
\change{Currently, there are 6 papers discussing on test selection and prioritization in ADS testing~\cite{kim2020reducing, wolschke2017observation, luo2021targeting, tang2021systematic, zhang2018deeproad, tian2018deeptest}}, while the SE community has investigated these two types of techniques quite a bit in traditional software testing~\cite{rothermel1996analyzing, zhang2018hybrid, busjaeger2016learning, elbaum2002test}. In traditional software testing, test selection aims to only select and re-run test cases affected by code changes, and test prioritization ranks test cases based on their likelihood of revealing failures. Traditional test selection and prioritization techniques rely on code coverage or program analysis (e.g., call graph analysis, dependency analysis) to measure the impact of code changes. However, traditional code coverage and program analysis techniques are not directly applicable to DL models.


% Furthermore, \textbf{coverage-based methods}~\cite{pei2017deepxplore, tian2018deeptest} are widely explored in the SE community. Coverage-based methods rely on the notion of neuron coverage~\cite{pei2017deepxplore} and its variants~\cite{ma2018deepgauge, hu2019deepmutation}. These methods assume that a test case with higher neuron coverage can expose more erroneous behaviors of a DNN model. DeepXplore~\cite{pei2017deepxplore} used a gradient-based search method to find inputs that maximize neuron coverage and cause inconsistent behaviors among multiple DNN systems. DeepTest~\cite{tian2018deeptest} used neuron coverage to identify road images that maximize erroneous behaviors of a driving model. 
% Harel-Canada et al.~\cite{harel2020neuron} showed that higher neuron coverage actually leads to fewer defects detected and less natural inputs. DeepRoad extended DeepTest to generate more natural road images using GAN~\cite{zhang2018deeproad}. Yet it need to be trained on a large amount of training data and is limited to simple transformations such as changing sunny weather to rainy weather. 

% The SE community should explore more advanced CV techniques such as~\cite{huang2018multimodal} to more effectively generate complex and realistic driving data. Moreover, existing work targets mainly at single-modal and simple end-to-end driving systems. As a future work, more systematic coverage-based research needs to be conducted to generate realistic driving scenes for multi-module and multi-modal ADSs.

% In recent years, several types of metrics are proposed for test selection or prioritization in DL models. In addition to \textbf{coverage-based metrics}~\cite{tian2018deeptest,zhang2018deeproad} (discussed in Section~\ref{sec:Need1GF}), 
%which has questionable correlation between neuron coverage and model robustness~\cite{harel2020neuron}, 
%\textbf{Coverage-based metrics}, such as neuron coverage~\cite{pei2017deepxplore} and k-multisection neuron coverage~\cite{ma2018deepgauge}
% , have been proposed to measure the coverage for DL models.

% In recent years, several types of metrics are proposed for test selection or prioritization in DL models. \textbf{Coverage-based metrics}~\cite{zhang2018deeproad, tian2018deeptest} are proposed to measure the coverage for DL models in End-to-End ADS. DeepTest~\cite{tian2018deeptest} has made use of neuron coverage to select newly generated road images to test autonomous driving models. DeepRoad~\cite{zhang2018deeproad} extended DeepTest to generate more natural road images using Generative Adversarial Networks. However, as discussed in~\cite{harel2020neuron}, the correlation between neuron coverage and model robustness is questionable. It is also unclear whether corner cases generated based on neuron coverage have practical significance in real-world ADS testing. For DL testing works in SE community, several techniques also present \textbf{confidence-based metrics}~\cite{feng2020deepGini, ma2021test, Li_2020PEACEPACT, wang2021prioritizing} to guide test selection and prioritization.

In recent years, several types of metrics are proposed for test selection or prioritization in DL models. \textbf{Confidence-based metrics}~\cite{feng2020deepGini, ma2021test, Li_2020PEACEPACT, wang2021prioritizing} are proposed to select or prioritize using the confidence (the output of the last hidden layer) of the DL model.
For example, DeepGini~\cite{feng2020deepGini} applied Gini impurity on confidence to measure the likelihood of misclassification on an input, and prioritized test cases with high Gini scores. In prior work, confidence-based metrics were applied to classification tasks, while an ADS contains many regression models. %~\cite{wang2021prioritizing} handled regression models by discretizing the output of a regression model and treated the regression model as a classification model. 
\change{PRIMA~\cite{wang2021prioritizing} uses mutation analysis to generate the handled regression models by discretizing the output of a regression model and treated the regression model as a classification model.} 
Then it performed small-scale mutations and trained a learning-to-rank-based ranking model to prioritize selected test cases. \change{Another type of testing metrics are \textbf{similarity-based test metrics}~\cite{luo2021targeting, tang2021systematic}. These methods select or prioritize test cases according to the similarity between the vector representation of each test cases. Similarly, likelihood-based surprise adequacy (LSA)~\cite{Kim_2019, kim2020reducing} and distance-based surprise adequacy (DSA)~\cite{wolschke2017observation} support embedding a test case using the output of a set of selected neurons. LSA measured the surprise of a test case by estimating the density of vector representations of each selected test case, while DSA used the Euclidean distance to calculate the ratio of the test case from its own class to other classes.}

% Another type of testing metrics are \textbf{similarity-based test metrics}~\cite{Li_2019Boosting, Zhou_2020Cost}.
% \todo{\cite{luo2021targeting, tang2021systematic} use scenario vector to calculate similarity or distance}
% \jz{todo:
% check the two papers, confirm their relevance to similarity-based test metrics
% }
% These techniques use the outputs of the last hidden layer to represent the distribution of test cases and select test cases that are most different from each other. Similarly, likelihood-based surprise adequacy (LSA)~\cite{Kim_2019, kim2020reducing} and distance-based surprise adequacy (DSA)~\cite{wolschke2017observation} support embedding a test case using the output of a set of selected neurons. LSA measured the surprise of a test case by estimating the density of vector representations of each selected test case, while DSA used the Euclidean distance to calculate the ratio of the test case from its own class to other classes. 



% Furthermore, the effectiveness of test selection and reduction methods was evaluated on image-based end-to-end driving models and promising results were reported ~\cite{Li_2019Boosting, wang2021prioritizing}. 
However, ADSs often contain multiple modules and take rich sensor data as input, rather than a single end-to-end model (Section~\ref{sec:ADStype}). Existing test selection or prioritization methods do not account for such multi-module architectures in ADSs. In future work, it is worth investigating how to embed multiple types of sensor data to analyze the similarity between driving scenes and filter repetitive ones. For example, researchers can design a new model to embed different types of sensor data altogether. On the other hand, instead of directly embedding sensor data, researchers can also leverage dynamic HD maps, which is an intermediate representation of driving scenes in an ADS. HD maps incorporate the outputs of perception models and are then fed as input for the following prediction and control modules. They can be used as a holistic representation for driving scenes. 

To account for multi-module architectures, researchers may want to investigate how to combine test metrics for inner model behaviors, such as neuron coverage and surprise adequacy, and logic-based test metrics, such as path coverage, to capture the interaction among multiple models, and interaction between models and logic-based control modules. One possible solution is to formulate this as a multi-objective optimization problem. A technique should search for a minimal set of test cases that collectively maximize the coverage of individual ML models as well as the path or dependency coverage of an ADS. For example, a driving scene at a busy traffic intersection is likely to have higher collective coverage at the model and system levels compared with a highway scene with little traffic, since it involves multiple types of objects (e.g., pedestrians, vehicles, and traffic lights) that may trigger multiple execution paths in an ADS and also trigger multiple perception models. Given the large number of possible test case combinations, it is worth investigating how to leverage multi-objective optimization algorithms to efficiently search for an optimal test set. 


\subsection{Gaps and Future Directions for Need 3}


%  Currently, there are two research directions in the SE community to automatically generate test cases for ADS testing: test case generation using real-world data and test case generation in simulation. For the first research direction, recently proposed approaches leverage on traditional image transformation method and DNN-based image generative method to generate new test cases based on the original dataset. In \cite{tian2018deeptest, zhang2018deeproad}, image transformations such as scaling, horizontal shearing, and rotation are used to simulate driving images collected by the camera being blocked, rotated, or in some extreme weather. For the DNN-based image generative method, Generative Adversarial Network (GAN)~\cite{gan} is applied to generate more authentic and complex driving images. In~\cite{zhang2018deeproad}, GAN was used to transform sunny driving images in the original dataset to driving images with heavy snow or hard rain, whose authenticity is significantly improved compared with traditional image transformation methods. These two kinds of approaches can quickly generate high-quality test scenarios based on real-world data. However, existing test case generation tools mainly focus on generating test cases in the form of the single-frame image, while current multi-module ADSs generally take images from multiple cameras deployed at different positions and other sensor data such as point clouds collected from LiDAR as inputs. This gap makes existing test case generation methods and tools proposed by academia less effective to test ADSs in the industry. Therefore, it implies great opportunities for researchers to study how to automatically generate multi-modality sensor data for testing multi-module ADSs. \ms{Need to move to Need 1}
% \titlebox{Future Direction 2:}{Develop test case generation tools for automatically generate multi-modality sensor data beyond images.}

% \todo{evidence that OpenScenario is dominate}
% For test case generation by simulation, as mentioned in Section~\ref{sec:simulation}, industry companies usually build testing scenarios in simulation by manually designing road networks, driving environment, and other settings related testing scenarios, it would take a large amount of time and resource to implement. Another approach is describing test scenarios in a DSL such as OpenScenario~\cite{OpenScenario} and GeoScenario~\cite{queiroz2019geoscenario}. Then the simulator can load the test scenario description and render corresponding test cases. However, existing DSLs usually have strict and complicated syntax. Writing testing scenario descriptions in DSL is also heavy. It would be better if there is a semi-automatic or automatic testing tool based on user instructions or written documents as mentioned in Section~\ref{sec:solve} and \ref{sec:unsolve}. The question is partially solved in~\cite{gambi2019generating}, where a method called AC3R was proposed to automatically simulate crash scenarios based on police reports. This method leverages NLP technologies to extract key information from police reports and then generate corresponding crash scenarios by a simulator. However, this method now can only simulate some simple crash scenarios such as rear-end collision of two vehicles. In real life, crash scenarios may be more complicated and involve multiple objects. It is still necessary to leverage the ability of DSL to define complicated testing scenarios. If there is a better DSL with the natural language syntax for abstracting test scenarios from human written documents and the DSL can be parsed by NLP technologies applied in~\cite{gambi2019generating}, more complicated testing scenarios can be automatically generated. In addition, the generation based on only text may not very accurate because other sources such as crash videos could provide more details of crashes. Applying a DSL to coordinate multiple sources of traffic records is also helpful for reconstructing complicated test scenarios. 

% For test case generation by simulation, as mentioned in Section~\ref{sec:simulation}, Domain Specific Languages (DSL), such as OpenScenario~\cite{OpenScenario} are used in simulation platforms to build the driving scenario and specify movement of traffic participants. However, as discussed in Section~\ref{sec:need3}, widely used DSLs are too strict in defining scenes and object motions, so that developers need to spend a lot of lines of code to define a simple overtaking scene. In order to make the development process more convenient, ADS developers need high-level DSL to automatically or semi-automatically build driving scenes, so as to avoid spending too much experience on unnecessary details.

As mentioned in Section~\ref{sec:simulation}, Domain Specific Languages (DSLs) are used by industrial practitioners to build driving scenarios and design participants' movement on simulators. However, as discussed in Section~\ref{sec:need3}, the current DSLs generally are limited by their usability: it is cumbersome to define scenes and object motions in those DSLs since it takes developers a lot of efforts (e.g., hundreds of lines of code) to even build simple ones.

% In SE community, a DSL, ADSML\cite{du2021towards}, was proposed to model statistic elements and entity actions of driving scenarios. And model generated by ADSML could be verified using UPPAAL-SMC. 
% \change{ADSML\cite{du2021towards}}基于MPS构建了面向自动驾驶领域的建模汽车自动驾驶场景中的静态元素和实体动态行为的DSL。并且构建的模型可以使用UPPAAL-SMC进行形式验证。

% 建模汽车自动驾驶场景中的静态元素和实体动态行为，通过实现一种面向汽车自动驾驶的领域特定
% 语言ADSML，支持用户在元编程系统MPS上创建汽车自动驾驶场景模型。

To reduce test construction effort, ADS developers wish the DSLs can flexibly express the semantics of the driving scenes without the necessity to specify all scene details.
%\change{In SE community, a DSL, ADSML\cite{du2021towards}, was proposed to model static objects and dynamic actions in a driving scene. In addition} \change{delete}, 
The Intelligent Vehicle community designed a few DSLs to achieve such goals~\cite{fremont2019scenic, queiroz2019geoscenario, althoff2017commonroad, bender2014lanelets}. For instance, Scenic~\cite{fremont2019scenic} is a probabilistic programming language which enables developers to generate complex traffic jam scenarios with just a few lines of code. These newly designed DSLs are more compact and flexible. However, they are rarely used by industry practitioners. One possible reason is that the languages are very costly to be adapted to existing simulators. This issue also exists in ML. To address it, ML practitioners proposed an open standard, Open Neural Network Exchange (ONNX), to help developers train and deploy models on different frameworks and hardware. Similarly, for ADS development and testing, creating a shared middleware can decouple simulators and DSLs and therefore reduce the effort of adapting new DSLs to existing simulators. 
%Currently, OpenScenario~\cite{OpenScenario}, as a standard of driving scenarios, has been widely supported by existing simulators, e.g., CARLA~\cite{carla}, CarMaker~\cite{CarMaker}, PreScan~\cite{prescan}, Cognata~\cite{Cognata}, Foretify~\cite{Foretify}, etc. In future work, the researcher may design OpenScenario-adaptive DSLs which can be supported by various simulators.
Currently, OpenScenario~\cite{OpenScenario}, as a standard of driving scenarios, has been widely supported by existing simulators including CARLA\footnote{\url{https://github.com/carla-simulator/carla}},
CarMaker\footnote{\url{https://ipg-automotive.com/products-services/simulation-software/carmaker/}}, 
PreScan\footnote{\url{https://tass.plm.automation.siemens.com/prescan-overview}},
Cognata\footnote{\url{https://cognata.com/closed-loop-simulations/}}, and
Foretify\footnote{\url{https://foretellix.com/technology/}}.
%, etc. 
In future work, %the researcher
researchers may design OpenScenario-adaptive DSLs, which can be supported by various simulators.



Furthermore, various forms of information can be utilized to guide driving scene construction, such as crash reports, videos, natural languages and flowcharts. %These forms can be viewed as hyper-DSLs which enrich the front end of middleware to boost development efficiency and flexibility. 
For example, in~\cite{gambi2019generating}, AC3R was proposed to automatically simulate crash scenarios via analyzing crash reports. This method leverages NLP techniques to extract key information (e.g., traffic participants and driving actions) from crash reports, transform crash information to a Lua script to control traffic participants and generate corresponding crash scenarios in simulator. AC3R is limited to some simple crash scenarios like rear-end collision of two vehicles. In addition, as crash reports often follow rigid narrative standards, AC3R may have a difficult time translating free-form driving scene descriptions to an executable driving scene. As future work, it is worth investigating new techniques in NLP and CV to support automated construction of driving scenes from text or video data.


% For test case generation by simulation, as mentioned in Section~\ref{sec:simulation}, Domain Specific Languages (DSLs) are used in simulation platforms to build the driving scenario and specify movement of traffic participants. However, as discussed in Section~\ref{sec:need3}, widely used DSLs are too strict in defining scenes and object motions, so that developers need to spend a lot of lines of code to define a simple overtaking scene. 

% In order to make the development process more convenient, ADS developers need high-level DSL to automatically or semi-automatically build driving scenes, so as to avoid spending too much time on unnecessary details. Currently, the intelligent vehicles community proposed few DSLs to solve this problem~\cite{fremont2019scenic, queiroz2019geoscenario, althoff2017commonroad, bender2014lanelets}. Scenic~\cite{fremont2019scenic} allows users to generate similar but slightly different scenes through the same code leveraging probabilistic programming language. And scenic can generate complex traffic jam scenarios with just a few lines of code. However, these new proposed DSLs are not widely used, because they need to be adapted to each existing simulator. To expand the application of new DSLs, a middleware that is widely adapted to existing simulators is needed. \change{For example, ONNX is a middleware to allow developers to transform their DL models on different DL platforms. The DSL middleware should play the same role.} By manipulating the middleware instead of a specific simulator, DSLs can be used on multiple simulators. Currently, OpenScenario~\cite{OpenScenario}, as a standard for driving scenarios, has been widely accepted by existing simulators, \change{such as CARLA~\cite{carla}, CarMaker~\cite{CarMaker}, PreScan~\cite{prescan}, Cognata~\cite{Cognata}, Foretify~\cite{Foretify}, etc.} \todo{supports}. In future work, new proposed DSLs could be compiled to OpenScenario to gain wildly application on simulators, and could focus on its expressive ability.

% \todo{ONNX}
% As future work, a middleware connecting the DSL and the simulator can be developed by SE community, as ONNX~\cite{} did for deep learning frameworks, to enable the new DSL to be supported by more simulators. 


% Furthermore, in order to improve the efficiency of generating driving scenes, external information can be used to guide the generation of driving scenes, such as crash reports, videos, natural language and flowcharts, which can be used as part of the front end of the middleware to assist DSL in building driving scenarios. 
% For example, in~\cite{gambi2019generating}, AC3R was proposed to automatically simulate crash scenarios based on police reports. This method leverages on NLP technologies to extract key information from police reports and then generate corresponding crash scenarios in a simulator. However, because AC3R did not convert extracted driving scenes to DSLs, it can only simulate some simple crash scenarios such as rear-end collision of two vehicles. In addition, the generation based on only text may not very accurate because other sources such as crash videos could provide more details of crashes. As future work, it is worth investigating how to leverage rich data to generate driving scenarios that could be complied by DSLs.

%现在的工业界怎么做的，现在的DSL是什么问题，但是工业界对现在用的dsl还不是很满意。

%现在学术界也提出了一些的DSL，但是并不能被广泛使用，主要问题是在DSL对simulator的兼容性上，需要很高的成本给DSL对simulator做适配。因此我们需要一个中间件来简化适配的成本。比如说openscenario，标准，比较广泛使用。学术界提出的dsl是否能compile成一个openscenario的文件？其次是openscenario是否还有值得优化的地方，从PL角度来看是否够简洁，表达能力如何，适配成本。
% \todo{ONNX: we have a same activation with ONNX, 介绍}

%USER对于DSL不满意，现在学术界提出来的工作 Scenic
%对于DSL来说，DSL能不能做的更加的userfriendly，支持多种形式的输入，比如自然语言，比如sketch（流程图生成，HCI），视频，构造更灵活的前端语言。然后把这个接到IR的前端。分析这写方法的缺陷，现在使用的NLP还是十分基础，只能用作生成简单的碰撞场景，流程图现在还没有被广泛的应用在这个领域



%我们需要一个compilor把dsl变异成IR或者是opensecnario

% To solve this problem, \todo{more cites} Scenic~\cite{queiroz2019geoscenario} refers to the probabilistic programming language, by imposing some constraints on the scene, sampling in the scene distribution to generate a specific driving scene. Therefore, Scenic allows developers to quickly define similar driving scenarios with the same code in batches. 
% However, because DSLs are usually bound to simulators, the new DSL can only support a small number of simlators, which makes it difficult for the new DSL to be promoted. As future work, a middleware connecting the DSL and the simulator can be developed by SE community, as ONNX~\cite{} did for deep learning frameworks, to enable the new DSL to be supported by more simulators. \todo{what these middleware can do}

% Furthermore, apart from the DSL, the SE and CV communities have also proposed some methods to automatically generate test scenarios based on videos or texts~\cite{}. For example, in~\cite{gambi2019generating}, AC3R was proposed to automatically simulate crash scenarios based on police reports. This method leverages on NLP technologies to extract key information from police reports and then generate corresponding crash scenarios by a simulator. 

% However, this method now can only simulate some simple crash scenarios such as rear-end collision of two vehicles. 
% In real life, crash scenarios maybe more complicated and involve multiple objects. In addition, the generation based on only text may not very accurate because other sources such as crash videos could provide more details of crashes. Therefore, the research on how to automatically reconstruct complicated test cases like crashes based on multiple source of traffic records is helpful for testing ADS.




% \todo{compiler,开发一个前段语言，把NLP或者ontologybased的方法或者建议的驾驶场景图来转换成openscenario}

% \todo{1. 现在每个dsl和simulator之间是紧密关联的，我们需要有一个每个平台通用的dsl来定义自动驾驶的场景作为前端，来联系到每个后端上去}

% \todo{1. 好写，但是适配的成本高，2. 适配的好，但是不好跟写。我们设计一个IR来链接两个方法}

% \todo{采访的时候发现不同的公司使用不同的simulator，需要用不同的dsl，对于好的dsl比如说scenic，他没办法应用在已有的simulator，使用openscenario来开发成本比较高}

% \todo{2.分析现有的dsl的pros and cons，有的灵活性差但是使用的多，有的灵活性好但是不好在simulator上使用，和中间表达很相似，我们能不能开发一个更精简的compilor，结合起来，把openscenario作为中间表示}

% \todo{大体思路：这是一个大的方向，其他社区的人做过部分工作，但是软工这边没有做}

% \todo{ONNX: we have a same activation with ONNX, 介绍}



% \todo{1.软工在这边的进展？没做的话，其他的社区做了一部分，他们的解决思路，}
% \todo{如何开发一个离用户更近的语言，现在openscenario不好使，我们怎么把好用的方法和opencsenario联合到一起}
% \todo{2. 现在这些思路的问题：结合？需要一个middleware。观察到学术界提出的}

% \todo{除了dsl以外，NLP，traffic-image也应该被用来生成test case}
% \todo{3. 需要一个更加flexable或者userfriendly的前端语言，可以基于NLP或者scratch，@几篇文章}


% \titlebox{Future Direction 3:}{Develop a better DSL to help generate test cases based on multiple source of traffic records.}

% Furthermore, how to automatically generate more test cases in simulation-based on existing ones has been also researched to improve ADS testing. In~\cite{Gambi_2019automatically}, a search-based testing method was proposed to change road networks and generate new test cases to detect potential defects of driving models in the simulated environment. In~\cite{han2020metamorphic}, a fuzz testing approach was proposed to randomly add noisy point clouds in the Baidu Apollo simulation environment to test ADSs. These approaches based on traditional search-based testing and fuzzing testing show that applying traditional testing approaches in simulation to generate new test cases is promising for improving ADS testing. It is worth further integrating such test methods in simulation. For example, fuzz testing can be applied to randomly change the surrounding environment such as the style of vehicles on road and buildings at the roadside. In this way, more test cases of different scenarios can be automatically generated. Another example is mutation testing~\cite{jia2010analysis}, which has been applied to evaluate the quality of test set in~\cite{hu2019deepmutation} by injecting errors into DL models. Though mutation testing is not a method for test case generation, the idea of error injection can be utilized for test case generation in simulation. By injecting faults such as breaking a camera or decreasing the signal magnitude of LiDAR, the rare situation in real life when an autonomous vehicle is broken can be simulated. In this condition, the robustness of ADSs against anomalous situations can be tested. \ms{not related, need to move to Need 1}

% \titlebox{Future Direction 4:}{Further investigate the application of traditional testing methods such as fuzz and mutation testing for test case generation in autonomous driving.}
% }


% \begin{comment}

% \subsubsection{Need 1: How to identify all possible corner cases and unexpected driving scenarios?}

% \lou{this paragraph should be discussed in need1 rather than 4.2.1}

% \todo{check}
% As discussed in section~\ref{sec:simulation_usage}, in industry, the mainly used solution to find corner cases is to extract driving scenes from real-world driving data and public driving datasets. However, these industrial methods still cannot find corner cases that rarely happens in real life.

% Currently, in SE community, the idea of generating and testing corner cases of ADS is similar to industry, relying on the driving experience and existing traffic laws to summarize corner cases. \cite{tian2018deeptest,zhang2018deeproad} test model behavior in extreme weather, camera contamination, and camera displacement. In~\cite{gambi2019automatically}, different road conditions are tested, such as passing intersections and roundabouts. In~\cite{gambi2019generating}, test cases are generated from accident crashing reports. 

% in SE community, several test adequacy \change{metrics} such as neuron coverage~\cite{pei2017deepxplore} and neuron boundary coverage~\cite{hu2019deepmutation} have been proposed for evaluating the quality of test sets for DL models. Such metrics are also used to guide the generation of new test cases that can achieve higher coverage of activated neurons. In SE community, test cases that can improve neuron coverage are considered as corner cases for DL models. For example, in DeepXplore~\cite{pei2017deepxplore}, corner cases were generated by maximizing neuron coverage to test E2E driving models. However, recent research argues that it is doubtful whether neuron coverage is meant to identify corner cases and test DL models~\cite{harel2020neuron}. In addition, generated test cases are more like adversarial examples~\cite{goodfellow2014explaining} that look similar to original test cases by adding human unperceived noises. Whether these corner cases are meaningful in the real-world is debatable. Furthermore, the mainstream multi-module ADS are more complicated than single DL models. It is also unclear whether generated corner cases targeting a DL model are still corner cases for industry-level ADS. Considering a real-world scenario of a corner case where a stop sign is damaged due to man-made or natural factor, whether it can be generated guided by neuron coverage metrics and whether it can trigger a mistake of a multi-module ADS? Therefore, it is worth investigating whether corner cases identified by neuron coverage adequacy or similar test metrics are meaningful in real world and whether they will cause mistakes in ADS.


% Although these methods have achieved better results in testing pre-defined scenarios, they still cannot cover corner cases as many as possible. The main problem is that there is no systematic approach to guide the identification of corner cases from diverse sources such as traffic rules and accident reports. \todo{This claim is not convincing. All previously mentioned approaches seem systematic to me. Also, \cite{gambi2019generating} generates test cases from crash reports. Why do you say there are no systematic approaches? Why diverse sources matter if we have good approaches for each source? We can just use those techniques in tandem.} Under this circumstance, {\color{blue}it is difficult to comprehensively summarize existing corner cases and identify new corner cases.} An actionable approach is to first construct a regulation list that covers a large number of existing corner cases derived from traffic rules and accident reports (e.g., National Highway Traffic Safety Administration traffic crash data~\cite{nhtsa}). Based on the regulation list, it is possible to summarize the common ground among identified corner cases and then create a domain specification language (DSL) to abstract characters of corner cases. \todo{Why is it hard if the benchmarks are already out there as you said in the next sentence?} Though several DSLs such as OpenScenario~\cite{OpenScenario} and GeoScenario~\cite{queiroz2019geoscenario} have been proposed, they only focus on the description and generation of test scenarios. Therefore, they cannot help identify which kind of corner cases should be generated. With the regulation-based DSL, it would be simpler to identify existing corner cases or even new corner cases.

% \titlebox{Future Direction 5:}{Propose a regulation-based DSL to help identify corner cases.\todo{Why is a new DSL a better solution? Why not automated test generation approaches?}}
 
% On the other hand, in SE community, several test adequacy \change{metrics} such as neuron coverage~\cite{pei2017deepxplore} and neuron boundary coverage~\cite{hu2019deepmutation} %is
% \change{have been} proposed for evaluating the quality of test sets for DL models. Such metrics are also used to guide the generation of new test cases that can achieve higher coverage of activated neurons. In SE community, test cases that can improve neuron coverage are considered as corner cases for DL models. For example, in DeepXplore~\cite{pei2017deepxplore}, corner cases were generated by maximizing neuron coverage to test E2E driving models. However, recent research argues that it is doubtful whether neuron coverage is meant to identify corner cases and test DL models~\cite{harel2020neuron}. In addition, generated test cases are more like adversarial examples~\cite{goodfellow2014explaining} that look similar to original test cases by adding human unperceived noises. Whether these corner cases are meaningful in the real world is doubtable. Furthermore, the mainstream multi-module ADS are more complicated than single DL models. It is also unclear whether generated corner cases targeting a DL model are still corner cases for industry-level ADS. Considering a real-world scenario of a corner case where a stop sign is damaged due to man-made or natural factor, whether it can be generated guided by neuron coverage metrics and whether it can trigger a mistake of a multi-module ADS? Therefore, it is worth investigating whether corner cases identified by neuron coverage adequacy or similar test metrics are meaningful in real world and whether they will cause mistakes in ADS.

%  \titlebox{Future Direction 6:}{Investigate the meaningfulness and effectiveness of generated corner cases guided by neuron coverage (or similar) test metrics in the real world.}

% \subsubsection{Need 4: How to automatically or semi-automatically generate test cases?} \todo{This need looks very similar/related to Need 1.}

% {\color{blue} Currently, there are two research directions in SE community to automatically generate ADS test cases: test case generation based on real-world data and test case generation in simulation. For the first research direction, recent proposed approaches leverage on traditional image transformation method and DNN-based image generative method to generate new test cases based on the original dataset. In \cite{tian2018deeptest, zhang2018deeproad}, image transformation such as scaling, horizontal shearing, and rotation are used to simulate driving images collected by the camera being blocked, rotated, or in some extreme weather. For the DNN-based image generative method, Generative Adversarial Network (GAN)~\cite{gan} is applied to generate more authentic and complex driving images. In~\cite{zhang2018deeproad}, GAN was used to transform sunny driving images in the original dataset to driving images with heavy snow or hard rain, whose authenticity is significantly improved compared with traditional image transformation methods. These two kinds of approaches can quickly generate high-quality test scenarios based on real-world data. However, existing research mainly focus on image generation. There is little research to generate continuous testing scenarios with multiple sensor data, while current multi-module ADS normally take images from multiple cameras deployed at different positions and other sensor data like point cloud collected from LiDAR as inputs. This gap makes existing test case generation methods proposed by academia less effective to test ADS in industry. Therefore, it is essential to research on test case generation for multiple sensor data.
% \titlebox{Future Direction 7:}{Investigate test case generation methods for multi-modal sensor data beyond images}

% For test case generation in simulation, as mentioned in Section~\ref{sec:simulation_usage}, industry companies usually build testing scenarios in simulation by manually designing road networks, driving environment, and other settings related testing scenarios, it would take a large amount of time and resource to implement.\todo{What you described here look very similar to Need 1.} In~\ref{need}, current industrial practitioners talked about they need a semi-automatic or automatic testing tool that could generate various driving scenarios according to user instructions or written documents. The question is partially solved in~\cite{gambi2019generating}, where a method called AC3R was proposed to automatically simulate crash scenarios based on police reports. This method leverages on NLP technologies to extract key information from police reports and then generate corresponding crash scenarios by a simulator. However, this method now can only simulate some simple crash scenarios such as rear-end collision of two vehicles. In real life, crash scenarios maybe more complicated and involve multiple objects. In addition, the generation based on only text may not very accurate because other sources such as crash videos could provide more details of crashes. Therefore, the research on how to automatically reconstruct complicated test cases like crashes based on multiple source of traffic records is helpful for testing ADS.

% \titlebox{Future Direction 8:}{Reconstruct test cases based on multiple source of traffic records.\todo{A better DSL seems to be a good solution for this goal.}}

% Furthermore, how to automatically generate more test cases based on existing test cases in simulation has been also researched to improve ADS testing. In~\cite{gambi2019automatically}, a search-based testing method was proposed to change road networks and generate new test cases that more likely detect potential defects of driving models in simulated environment. In~\cite{han2020metamorphic}, a fuzz testing approach was proposed to randomly add noisy point clouds in Baidu Apollo simulation environment to test ADS. These approaches based on traditional search-based testing and fuzzing testing show that applying traditional testing approaches in simulation to generate new test cases is promising for improving ADS testing. It is worth further integrating such test methods in simulation. For example, fuzz testing can be applied to randomly change the surrounding environment such as the style of vehicles on road and buildings at roadside. In this way, more test cases of different scenarios can be automatically generated. Another example is about mutation testing~\cite{jia2010analysis}, which has been applied to evaluate the quality of test set in~\cite{hu2019deepmutation} by injecting errors into DL models. Though mutation testing is not a method for test case generation, the idea of error injection can be utilised for test case generation in simulation. By injecting faults like breaking a camera or decreasing the signal magnitude of LiDAR, the rare situation in real life when an autonomous vehicle is broken can be simulated. In this condition, the robustness of ADS against anomalous situation can be tested.

% \titlebox{Future Direction 9:}{Apply traditional testing methods such as fuzz and mutation testing for test case generation.\todo{This is vague. Isn't people doing this? What's new in this direction?}}
% }

% \end{comment}


% There are three commonly used methods in the current software engineering academic community to generating ADS test cases: traditional image transformation method, DNN-based image generative method, and simulator-based test case generation method. For traditional image transformation methods, traditional computer vision methods are used to generate new driving images from the original dataset. In \cite{tian2018deeptest, zhang2018deeproad}, scaling, horizontal shearing, and rotation are used to simulate driving images collected by the camera being blocked, rotated, or in some extreme weather. For the DNN-based image generative method, Generative Adversarial Network (GAN) is used to generate more authentic and complex driving images. In~\cite{zhang2018deeproad}, GAN is used to transform sunny driving images in the original realistic driving dataset to heavy snow and hard rain driving images, whose authenticity is significantly improved when compared with traditional image transformation methods. In~\cite{zhou2018deepbillboard}, adversarial attack in the physical world is investigated. A new test set is generated by replacing billboards in driving scenes with adversarial noises to test the robustness of autonomous driving systems. Comparing with driving images generated by traditional methods, adversarial images generate in~\cite{zhou2018deepbillboard} are more likely to find vulnerabilities in ADS. The above research directly generates test scenarios on images collected in the real world, while other work construct test scenarios in simulated environments. For example, In~\cite{gambi2019automatically}, various virtual roads are generated in a simulator called BeamNG.research to test whether an autonomous driving system could keep running along the road lane. In~\cite{gambi2019generating}, a method called AC3R is proposed to simulate crash scenarios based on police reports. 

% The first two approaches can quickly generate high-quality test scenarios based on real-world data. However, these two methods only focus on image data for a single frame and it is difficult to generate continuous scenarios and data with multiple sensors, which limits the type of driving scenarios that this method can test. Compared with the first two approaches, the simulator-based approach has the potential to generate multiple sensors and continuous driving scenarios, while its authenticity has always been questioned.

% As discussed in section~\ref{need}, current industrial practitioners need to have a semi-automatic testing tool, which consists of two parts: one can generate various driving scenarios that users want in batches according to user instructions or written documents. The other is an automated testing process, including user instruction analysis, test case generation, and test result evaluation.
% Although existing software engineering research in ADS testing can generate specific test cases, most of these test cases rely on manual design and cannot be generated in batches. In practical applications, written documents such as traffic accident reports, traffic laws, and industry standards often record dangerous driving scenarios and driving guidelines, which will be used as references when manually designing test cases. Therefore, if there are tools that can extract test cases from these written documents and reconstruct them in a simulation environment, the labor cost of generating test scenarios can be reduced. \lou{deviates from the main idea} 
% \titlebox{Future Direction 3:}{Reconstruct test cases based on traffic scenes records.}

% Secondly, fuzzing testing and mutation testing commonly used in traditional software engineering can also generate driving scenarios that users need in batches according to user requirements. \change{Currently, few works in SE community apply fuzzing testing and mutation testing to deep learning testing.} \cite{guo2018dlfuzz} is the first work to use differential fuzzing testing to test image classification, deep learning model. This research treats the goal of achieving higher neuron coverage and exposing more abnormal behaviors as a joint optimization problem and uses a series of mutation strategies to perturb the input image to achieve higher neuron coverage. In \cite{hu2019deepmutation}, DeepMutation was proposed to be used in image classification deep learning models for mutation testing. Compared with \cite{guo2018dlfuzz}, DeepMutation not only mutates the data such as noise disturbance and data loss but also performs mutation tests at the program level and the model level, such as randomly deleting a layer of DNN or swapping two neurons in a layer. \todo{Add connection sentence} These two techniques can be integrated into simulation to automatically generate more test cases. For example, by randomly changing the environment like the style of vehicles on road and surround buildings, more testing cases can be obtained. The mutation testing technique can be used to inject faults into ADS in the simulation environment and then create testing scenarios to evaluate whether ADS is robustness enough to work normally under these scenarios.
% \titlebox{Future Direction 4:}{Apply fuzzy and mutation testing for test case generation.}


% In addition, it should be noted that the current test case production methods of SE community mainly focus on the generation of camera-based test cases. These test cases cannot fully test ADS that uses multiple sensors in the industry. In future work, ADS test case generation needs to consider multi-modality and multi-sensor, especially in metamorphic testing, the data of multiple sensors may need to be transformed at the same time.
% \titlebox{Future Direction 5:}{Propose a testing tool to generate multi-modality test cases for autonomous driving system.}


% As discussed in section~\ref{need}, current industrial practitioners need to have a semi-automatic testing tool, which consists of two parts: one can generate various driving scenarios that users want in batches according to user instructions or written documents. The other is an automated testing process, including user instruction analysis, test case generation, and test result evaluation. Although existing software engineering research in ADS testing can generate specific test cases, most of these test cases rely on manual design and cannot be generated in batches. 

% \change{In practical applications, there are many resources that can be used as the basis for designing test cases. For example, written documents such as traffic accident reports, traffic laws and industry standards often record dangerous driving scenarios and driving instructions. In~\cite{gambi2019generating}, a method is proposed to simulate crash scenarios based on police reports. In addition, traffic accident videos recorded by CCTV traffic cameras and driving recorders can also be used to generate test cases. CADP~\cite{shah2018cadp} includes 1,416 traffic accident video clips collected from YouTube \todo{find another example}. By modifying or remodeling this data set, traffic accident test cases can be generated in batches.}
% \titlebox{Future Direction 3:}{Reconstruct test cases based on traffic scenes records.}

% Secondly, fuzzing testing and mutation testing commonly used in traditional software engineering can also generate driving scenarios that users need in batches according to user requirements. Currently, there are some works that apply fuzzing testing and mutation testing to deep learning testing. \cite{guo2018dlfuzz} is the first work to use differential fuzzing testing to test image classification, deep learning model. This research treats the goal of achieving higher neuron coverage and exposing more abnormal behaviors as a joint optimization problem and uses a series of mutation strategies to perturb the input image to achieve higher neuron coverage. In \cite{hu2019deepmutation}, DeepMutation was proposed to be used in image classification deep learning models for mutation testing. Compared with \cite{guo2018dlfuzz}, DeepMutation not only mutates the data such as noise disturbance and data loss but also performs mutation tests at the program level and the model level, such as randomly deleting a layer of DNN or swapping two neurons in a layer. \todo{Add connection sentence} These two techniques can be integrated into simulation to automatically generate more test cases. For example, by randomly changing the environment like the style of vehicles on road and surround buildings, more testing cases can be obtained. The mutation testing technique can be used to inject faults into ADS in the simulation environment and then create testing scenarios to evaluate whether ADS is robustness enough to work normally under these scenarios.
% \titlebox{Future Direction 4:}{Apply fuzzy and mutation testing for test case generation.}

% In addition, There are three commonly used methods in the current software engineering academic community to generating ADS test cases: traditional image transformation method, DNN-based image generative method, and simulator-based test case generation method. For traditional image transformation methods, traditional computer vision methods are used to generate new driving images from the original dataset. In \cite{tian2018deeptest, zhang2018deeproad}, scaling, horizontal shearing, and rotation are used to simulate driving images collected by the camera being blocked, rotated, or in some extreme weather. For the DNN-based image generative method, Generative Adversarial Network (GAN) is used to generate more authentic and complex driving images. In~\cite{zhang2018deeproad}, GAN is used to transform sunny driving images in the original realistic driving dataset to heavy snow and hard rain driving images, whose authenticity is significantly improved when compared with traditional image transformation methods. In~\cite{zhou2018deepbillboard}, adversarial attack in the physical world is investigated. A new test set is generated by replacing billboards in driving scenes with adversarial noises to test the robustness of autonomous driving systems. Comparing with driving images generated by traditional methods, adversarial images generate in~\cite{zhou2018deepbillboard} are more likely to find vulnerabilities in ADS. The above research directly generates test scenarios on images collected in the real world, while other work construct test scenarios in simulated environments. For example, In~\cite{gambi2019automatically}, various virtual roads are generated in a simulator called BeamNG.research to test whether an autonomous driving system could keep running along the road lane. In~\cite{gambi2019generating}, a method is proposed to simulate crash scenarios based on police reports.

% In addition, it should be noted that the current test case production methods of SE community mainly focus on the generation of camera-based test cases. These test cases cannot fully test ADS that uses multiple sensors in the industry. In future work, ADS test case generation needs to consider multi-modality and multi-sensor, especially in metamorphic testing, the data of multiple sensors may need to be transformed at the same time.
% \titlebox{Future Direction 5:}{Propose a testing tool to generate multi-modality test cases for autonomous driving system.}



% \subsection{Needs that have not been addressed by the SE community}
% \label{sec:unsolve}
% \todo{Add connection sentence}





\begin{comment}
\subsection{Need 3: How to improve the authenticity of the simulation environment?}
% In the current ADS testing process, simulation testing is an important step. However, the authenticity of simulation tools is always questioned by industrial. The authenticity of simulation tools includes two aspects. The first one is the authenticity of simulated sensor data, such as whether the data generated by multiple sensors match each other, and whether the generated data meets the physical rules. It is for the consideration of the authenticity of simulation data that some industrial participants test ADS under extreme weather conditions in reality, instead of relying solely on simulation tools to test the performance of ADS under extreme weather conditions. The second one is the authenticity of the autonomous vehicle in the simulation platform. In real-life automatic vehicles, there are delays in the steps of generating and executing driving instructions due to data transmission and algorithm operation, but this is rarely reflected in models of automatic vehicles in the simulation environment. In addition, the power transmission, chassis, and other key components of vehicles have not been realized on all simulation platforms. This will cause ADS to make the following behaviors in the simulation environment that do not conform to the actual physical environment.
% In the current 
Simulation plays an important role in ADS testing, however, the authenticity of the simulation environment is always questioned %by industrial
in industry. The lack of authenticity is mainly performed as the texture of rendered images looks not realistic as the real world. Because currently DL models deployed in ADSs are trained on real-world datasets, the difference between the rendered scenarios and real-world scenarios may cause unexpected impacts on testing. For example, some defects identified in a simulation environment may be caused by the difference coincidentally and these defects cannot be reproduced in on-road testing. 
For the SE community, it is difficult to directly solve the problem by improving simulation environments. However, why the lack of authenticity would influence the testing is a question worth researching comprehensively. Unlike traditional software testing where the quality of input can be systematically measured by several metrics such as code coverage~\cite{tikir2002efficient} and statement coverage~\cite{yang2009survey}, it is unclear how to measure the quality of input for DL models. Though some work such as neuron coverage~\cite{pei2017deepxplore} was proposed, they did not consider the relationship between the authenticity and the quality of test cases. For example, when images with different resolutions originating from the same source image are fed into a DL model, the predictions may be different. In this condition how can we validate the quality of test inputs and test results? If we can analyze the question clearly, we could better make use of testing results in simulation even if there exist authenticity problems.      

% \titlebox{Future Direction 6:}{Investigate how to validate test input for DL components.}


Similarly, in addition to the authenticity of data, compared with the real world, the authenticity of the model in simulation is also worth studying. For example, hardware delays and errors in the simulation platform are often ignored, but in real-world practice, the accumulation of delays and errors will cause the performance of ADSs to be not as good as in the simulation test. In order to reduce the impact of the simulation authenticity of models on testing, hardware-in-the-loop testing is a promised method. Hardware-in-the-loop (HIL) testing \cite{bullock2004hardware} is a simulation test involving actual hardware components. In the autonomous driving test, the hardware-in-the-loop test allows the actual hardware components of the autonomous vehicle (such as powertrain and chassis) to interact with the virtual vehicle model in the simulation platform, and to simulate the performance of ADSs in actual deployment situations. There are many studies on the HIL of ADS. \cite{joshi2017powertrain} develops a HIL simulator to link the powertrain and chassis of the ego-vehicle, and compared the real-time performance of the ego-vehicle with the real-time performance of HIL simulation. \cite{chen2018autonomous} links the HIL with the electronic control unit for hardware control to test scene perception, path planning, decision-making, and vehicle control algorithms. In \cite{gietelink2006development}, the entire ego-vehicle was configured into HIL, rather than the powertrain to test its adaptive cruise function and forward collision warning function. In future work, how to combine HIL with existing testing methods, such as metamorphic testing and fuzzing testing, to build a more flexible and automated testing program can be a research direction.

% \titlebox{Future Direction 7:}{%How to combine Hardware-in-the-loop with existing testing methods?
% %Combine the Hardware-in-the-loop with existing test methods to avoid authenticity problems.
% Combine the Hardware-in-the-loop with existing testing methods to avoid deviations caused by unrealistic hardware in simulation testing.
% }
\end{comment}

% \titlebox{Future Direction 7:}{Use metamorphic testing to reduce the impact of simulation accuracy problems on testing.}

% Now SE community seldomly use simulation tool to test autonomous driving systems.
% How to take advantages of simulation to test autonomous driving systems more comprehensively.
% How to efficiently define and build test scenarios using DSL.
% How to efficiently import test scenarios (e.g., accident report) into simulation
% How to improve test quality in simulation testing
% How to create an authentic and complicated simulation environment
% How to evaluate the test quality in simulation. 


% \todo{paper: Evaluating Validity of Synthetic Data in Perception Tasks for Autonomous Vehicles}


% \todo{Therefore,ADS developers wish to get more tool support to analyze, recognize,and repair labeling errors in their driving data.}

\subsection{Gaps and Future Directions for Need 4}
% \change{currently, 


% manually generate oracle for driving data }

Currently, industrial practitioners need to manually collect, clean, and label raw sensor data for training and testing ADSs. As discussed in Section~\ref{sec:need4}, they wish to have more tool support for this process. In general, data collection, cleaning, and labeling are crucial steps in the development pipeline of AI-based applications, which has been recognized as an important research area by the SE community~\cite{amershi2019software}. However, we only find several SE work related to this direction in the literature survey. There is much more SE researchers can potentially contribute to.   

% 1. based on test result, recommend which data (e.g., video clips or road images) to label first. 
% 2. intelligent auto-labeling 

% 分成两个问题：auto labeling, data clearning
% 1. 
% 2.clearning: Assessing the Impact of Automated Suggestions on Decision Making: Domain Experts Mediate Model Errors but Take Less Initiative



%During the on-road testing, as various sensors are equipped in autonomous vehicles, it is common that the collected data are not synchronized perfectly due to sensor delays. 

SE researchers can develop automated or semi-automated tool support to reduce data labeling effort. Test selection and prioritization techniques can be applied to recommend which tests need to be labeled first. In the SE community, Kim et al.~\cite{kim2020reducing} proposed to reduce data labeling effort using surprise adequacy~\cite{Kim_2019}. 
Other communities such as database and computer vision have proposed several supervised or semi-supervised learning techniques for automatically generating data labels~\cite{benato2021semi, ke2019end, chen2014beat, wu2018tagging, ke2017data, chen2013fast}. 
% ke2019end通过CNN来进行端到端自动标注，并且用ML-WGAN来增强数据并提升CNN的泛化能力。
% benato2021semi使用了半监督的方式进行标注。首先先用autoencorder将输入编码成特征，然后再在特征空间上将小部分标记好的数据的标签，传播给未被标记的数据。
% chen2014beat利用 3D 信息在给定带注释的 3D 边界框的情况下自动生成非常准确的对象分割。
We suggest readers to refer to Roh et al.~\cite{roh2019survey} for a detailed survey of data collection and labeling tools built by other research communities. The Human-Computer Interaction community has also explored how to provide better support for data labeling via crowdsourcing~\cite{wauthier2011bayesian, kazai2013analysis, bragg2013crowdsourcing, nowak2010reliable}. It would be interesting to investigate how to synergize those techniques from different communities to achieve more effective data labeling. 

% Furthermore, the SE a

% Multi-modal sensor data => label one type of sensor data, automatically populate to other types of data

% \cite{feng2020deepGini, ma2021test, Li_2020PEACEPACT, wang2021prioritizing, Li_2019Boosting, Zhou_2020Cost, Kim_2019, Kim_2020, wolschke2017observation}

% \cite{feng2020deepGini, Li_2019Boosting}


Furthermore, the SE community can contribute to data cleaning by developing input validation or outlier detection techniques on driving data. Traditional data cleaning approaches rely on users to provide a set of specific rules to determine constraints~\cite{gudivada2017data, chu2016data, rahm2000data}. Such rules are easy to define on tabular data or text data. However, it is challenging to define such rules for sensor data such as videos and point clouds that involve complex driving scenes. The SE community has proposed many techniques to identify failure-inducing inputs in software testing and debugging~\cite{zeller2002simplifying, misherghi2006hdd, clause2009penumbra, gulzar2016bigdebug, sun2018perses, gopinath2020abstracting, barowy2014checkcell}. For example, Gulzar et al.~\cite{gulzar2016bigdebug} leveraged data provenance to trace error propagation in big data systems and identify fault-inducing data. It would be beneficial to investigate how to adapt or renovate these techniques to identify low-quality data that leads to abnormal driving behavior in ADSs.

%Overall, there are many open problems and challenges in this domain. We believe the SE community can bring a unique angle and contribution to the research on data collection, labeling, and cleaning in autonomous driving testing.

%%%
%1. how to use model behavior analysis, test selection and prioriatization to recommend which data to label first
%2. automated data labeling for multi-modal sensor data
%3. failure inducing input analysis for data cleaning, i.e., removing low-quality data


%To solve these two problems together, developing middleware that contains both data validation and processing functionalities seems promising. In~\cite{emmerich2000software}, middleware was seen as a solution for heterogeneity and communication problems in distributed systems. In ADS, the heterogeneity problem of data can be solved by similar middleware. In~\cite{nikzad2014ape}, middleware was used to coordinate multiple operations across a mobile application, which leads to the possibility of using middleware to manage data validation and processing in ADS. With the middleware, it will be more convenient to obtain high-quality data for validating and testing ADS, which is worth investigation.
%Therefore, it is worth investigating middleware for data validation and processing in future work.

%\titlebox{Future Direction 8:}{Develop middleware for data validation and processing to help obtain high quality test data.}



==> Paper_Sections/backup_need1.tex <==
\subsection{Gaps and Future Directions for Need 1}
\label{sec:Need1GF}
Corner cases in ADSs are thought as safety-critical driving scenarios that are rare in the real world and possibly cause traffic accidents (e.g., collision).
As discussed in section~\ref{sec:need1}, %in industry, 
the de facto way to find corner cases in the industry is to conduct long hours of on-road testing.
However, this method is time-consuming and expensive.

The SE community has investigated a variety of methods to generate corner cases for ADSs. One common method is \textbf{search-based testing} %\cite{kluck2019genetic, Ben_Abdessalem_2016testing, abdessalem2018testing, Gambi_2019automatically, Calo_2020generating, cal2020simulaneously, han2020metamorphic, li2020avfuzzer, mullins2018adaptive, riccio2020model, Abdessalem_2018testing, Gladisch_2019experience}.
\change{\cite{gambi2019asfault, luo2021targeting, tang2021systematic, gladisch2019experience, ishikawa2020testing, borg2021digital, yin2021analyzing, laurent2021achieving, coletti2021diagnosing, calo2020simultaneously, abdessalem2018vision, gambi2019automatically}}
Search-based testing aims to find a set of testing parameters in a parameter search space to simulate testing scenarios that are most likely to cause collision. 
The search process is normally guided by manually defined fitness functions such as time-to-collision and minimal distance between the ego-vehicle and pedestrians. Optimal solutions of such fitness functions are usually found by applying genetic algorithms~\cite{Ben_Abdessalem_2016testing}. These methods require prior knowledge to define a proper search space and fitness function. Given the variety and complexity of real-world driving scenarios, it is challenging to pre–define a tractable search space. It is also challenging to search for the unknowns. Wang et al.~\cite{wang2020automatic} explored how to mine new requirements and corresponding formal constraints from use case specifications using NLP techniques for cyber-physical systems. Gambi et al.~\cite{gambi2019generating} explored how to generate driving scenarios from historical crash reports. As a future direction, it is worth investigating how to elicit new safety requirements from existing crash reports, traffic rules and on-road driving recordings. Such requirements can be used to generate new fitness functions or refine existing ones to augment the search space for more mission-critical testing scenarios. 
%augment a pre-defined search space with new test data, e.g., new on-road driving recordings. %More importantly, the test cases generated might be used in a closed-loop to elicit more useful requirement and generate more safety-critical test cases for autonomous vehicles.

Another type of corner cases generation explores the {\bf adversarial space} from existing testing data to mislead a model to make wrong predictions~\cite{goodfellow2014explaining, szegedy2013intriguing}. Wang et al.~\cite{wang2021advsim} used a new adversarial cost function to apply perturbations on input data to generate collision-prone trajectories. The cost function combines a trajectory cost, a collision cost and a safety cost to generate adversarial trajectories for a multi-module driving system. These unsafe trajectories are then implemented by modifying existing real LiDARs sweeps to generate feasible collision scenarios. Similarly, Mouret et al.~\cite{mouret2015illuminating} presented an approach that utilizes illumination search to identify an optimal feature map. This feature map is then used to generate corner cases to test a lane keeping assistant system. These methods require either prior knowledge to define the required evaluation metrics (e.g, standard deviation of the steering angle) or are restricted to single-modal sensor (LiDAR). As future work, new {\bf adversarial space} search algorithms are needed to allow exploring dangerous traffic scenarios with multi-modal sensor input data~\cite{daab2019feature, li2019aads}. Another promising line of work is to use geometry-aware adversarial cost function to generate corner-case scenarios, which is more suitable for the underlying sensor data~\cite{wen2019geometry}.

%new {\bf adversarial space} search algorithms are needed  algorithms for searching the 
%selection of feature vectors can be automated by using those search algorithms more suitable for the underlying geometric nature (e.g., feature vectors)~\cite {} and multi-modal sensor input data~\cite{daab2019feature}.



%{\bf adversarial space}, which applies perturbations on input data to mislead a model to make wrong predictions~\cite{goodfellow2014explaining, szegedy2013intriguing}. Wang et al.~proposed a new adversarial cost function, which combines a trajectory cost (i.e., the deviation from the safe trajectory), a collision cost, and a safety cost (e.g., high acceleration) to select adversarial trajectories~\cite{wang2021advsim}. These unsafe trajectories are then reflected by modifying existing real LiDAR sweeps to generate feasible collision scenarios.
%One future direction following this line of work is to generate corner-case scenarios consisting of multiple sensors instead of LiDAR. One possible solution is to generate test inputs with multiple sensors directly by finding adversarial examples in the input feature space of an end-to-end driving system but with a multi-module structure~\cite{casas2021mp3}.
%Another similar work utilizes illumination search~\cite{mouret2015illuminating}, which is able to illuminate the optimal solution surface in a feature space specified by users, to explore the feature space to identify the feature map (combination of feature vectors) which can mislead a lane keeping assistant system~\cite{zohdinasab2021deephyperion}. Such interpretable feature map can be used to generate corner-case test inputs. One possible future direction is to automate the selection of feature vectors (e.g., smoothness of the road) and evaluation metrics (e.g., standard deviation of the steering angle) based on relevant information learned from available crash report or explore the feature space using search algorithms more suitable for the geometric nature (e.g, feature vectors and linear transformations) or the underlying multi-modal sensor data~\cite{daab2019feature}.

Furthermore, \textbf{coverage-based methods}~\cite{pei2017deepxplore, tian2018deeptest} are widely explored in the SE community. Coverage-based methods rely on the notion of neuron coverage~\cite{pei2017deepxplore} and its variants~\cite{ma2018deepgauge, hu2019deepmutation}. These methods assume that a test case with higher neuron coverage can expose more erroneous behaviors of a DNN model. DeepXplore~\cite{pei2017deepxplore} used a gradient-based search method to find inputs that maximize neuron coverage and cause inconsistent behaviors among multiple DNN systems. DeepTest~\cite{tian2018deeptest} used neuron coverage to identify road images that maximize erroneous behaviors of a driving model. 
%Though this line of work has also been extensively studied~\cite{Gopinath_2018DeepSafe}, 
Harel-Canada et al.~\cite{harel2020neuron} showed that higher neuron coverage actually leads to fewer defects detected and less natural inputs. DeepRoad extended DeepTest to generate more natural road images using GAN~\cite{zhang2018deeproad}. Yet it need to be trained on a large amount of training data and is limited to simple transformations such as changing sunny weather to rainy weather. The SE community should explore more advanced CV techniques such as~\cite{huang2018multimodal} to more effectively generate complex and realistic driving data. Moreover, existing work targets mainly at single-modal and simple end-to-end driving systems. As a future work, more systematic coverage-based research needs to be conducted to generate realistic driving scenes for multi-module and multi-modal ADSs.
%~\cite{casas2021mp3}. 

